Clinical Trial Active Learning

This paper presents a novel approach to active learning that takes into account the non-independent and identically distributed (non-i.i.d.) structure of a clinical trial setting. There exists two types of clinical trials: retrospective and prospective. Retrospective clinical trials analyze data after treatment has been performed; prospective clinical trials collect data as treatment is ongoing. Typically, active learning approaches assume the dataset is i.i.d. when selecting training samples; however, in the case of clinical trials, treatment results in a dependency between the data collected at the current and past visits. Thus, we propose prospective active learning to overcome the limitations present in traditional active learning methods and apply it to disease detection in optical coherence tomography (OCT) images, where we condition on the time an image was collected to enforce the i.i.d. assumption. We compare our proposed method to the traditional active learning paradigm, which we refer to as retrospective in nature. We demonstrate that prospective active learning outperforms retrospective active learning in two different types of test settings.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Sections/intro_v1.tex <==
Clinical trials are research studies that evaluate the effects of medical treatments \cite{chien2022multi}. There are two different types of clinical trials: retrospective and prospective as illustrated in Figure \ref{fig:retro_vs_prosp}. In part a) of Figure \ref{fig:retro_vs_prosp}, a retrospective clinical trial collects data about participants after treatment has been administered. A retrospective clinical trial has access to the entirety of the pre-existing data and has no control over the design of the clinical trial itself. However, part b) of Figure \ref{fig:retro_vs_prosp} shows that a prospective clinical trial collects data about participants over time as they are receiving treatment \cite{euser2009cohort}. Prospective clinical trials are designed with a specific treatment and research plan, and only data collected throughout the clinical trial is used for analysis.

In the case of ophthalmology, an example of a prospective clinical trial is illustrated in Figure \ref{fig:clinical}. In part a) of Figure \ref{fig:clinical}, the patient is assessed by a doctor at each visit. During this visit, the patient is examined, as shown in part b), and clinical values such as Best Corrected Visual Acuity (BCVA) and central subfield thickness (CST) are obtained. Then, diagnostic imaging, such as Optical Coherence Tomography (OCT), is collected from the patient. Using the collected information, the doctor recommends a treatment plan to manage Diabetic Retinopathy (DR) or Diabetic Macular Edema (DME), demonstrated in parts c) and d) of the figure. Finally, in part e) the patient follows up with the doctor after a few weeks to reassess the status of the disease. Throughout this process, data collected at each visit from a patient is dependent on factors from that patient's previous visits, mainly whether treatment was administered and how long the patient waits between successive visits.
\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{PAPER/Figures/retro_vs_prosp.png}
\caption{Retrospective vs Prospective Clinical Trial Description}
\label{fig:retro_vs_prosp}
\end{figure}
%The main complication is due to how difficult it is for doctors to interpret the existence and status of a disease, especially given the large volume of patients doctors assist during a given day. 

The procedure illustrated in Figure \ref{fig:clinical} has many complications. The main complication is that doctors assist a large volume of patients on any given day. This demand is demonstrated in a study from 2015 \cite{mcdonald2015effects} which concluded that the average radiologist is tasked with interpreting an image every 3-4 seconds to satisfy their large workload, which is typically not possible due to how time-consuming and difficult it is to interpret these images. This increased workload leads to burnout, fatigue, and a large labeling error rate.

Thus, to alleviate these complications, machine learning is a potential solution to assist doctors through many of the steps listed in Figure \ref{fig:clinical} of a clinical trial. Machine learning identifies meaningful features from data automatically, allowing model outputs to provide a second opinion to doctors when diagnosing patients for certain diseases \cite{wang2017chestx}, \cite{wu2019deep}.

% In Figure \ref{fig:clinical}, the labeling task is eye disease classification, which affects treatment decisions and overall patient health. Given how crucial it is for medical data to be properly labeled and diagnosed, machine learning algorithms can be considered as a solution to automate many of the steps listed in Figure \ref{fig:clinical} of a clinical trial. Machine learning identifies meaningful features from data automatically, translating to completing labeling tasks at a persistent rate, unlike what is possible for human annotators. To support machine learning's potential, there has been a history of machine learning algorithms being applied successfully in the medical field, from detecting thoracic diseases in chest x-rays \cite{wang2017chestx} to screening for breast cancer \cite{wu2019deep}.
However, most standard machine learning algorithms require large amounts of labeled data samples in order to accurately train a model. In the medical field, this labeled data, as stated previously, is oftentimes time-consuming and challenging to provide. In addition, many labels can only be provided by trained medical professionals. Active learning is a common approach to tackle this issue. Active learning does not require a large labeled set; instead, it selects a subset of training samples to label and train with. Active learning uses query strategies to acquire this new selection of data and provide it to an external oracle for labeling, reducing the overall amount of data examined and annotated by an expert while still achieving high accuracy \cite{settles2009active}. The query strategies aim to select the most informative samples, resulting in a refined training set that quickly reduces the generalization error \cite{kumar2020active}. 

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{PAPER/Figures/clinical_trial_new.png}
    \caption{Clinical trial setup for DR/DME treatment}
    \label{fig:clinical}
\end{figure*}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{PAPER/Figures/CHANGE_in_clinical.png}
    \caption{Change in average BCVA and CST reported in patients across visits}
    \label{fig:change_clinical}
\end{figure}
% critical statement of AL first
While active learning bypasses the need for large amounts of labeled data, prior query strategies assume that the data is independent and identically distributed (i.i.d), as data is sampled based solely on a query criteria \cite{settles2009active}, \cite{wang2015querying}. Traditional attempts to use active learning do not assume dependencies that occur during the data collection process, such as the treatment and time dependencies present in Figure \ref{fig:clinical}. Thus, these traditional attempts can be considered as viewing the active learning process from a retrospective lens \cite{logan2022decal}, \cite{smailagic2018medal}.
% focus on the problem through a retrospective lens such as in \cite{logan2022decal}, \cite{smailagic2018medal}, and there have been limited attempts to view machine learning from the prospective clinical trial lens illustrated in Figure \ref{fig:clinical}. 

However, there are several issues with the i.i.d. assumption most active learning approaches take: 1) it disregards the non-i.i.d. dependencies and consequences of these dependencies that arise during the clinical trial collection procedure and 2) it does not mirror how the data collection process is realistically performed. Following the first point, this is easily observed by examining Figure \ref{fig:clinical}, where patients sometimes receive treatment at each visit. Therefore, due to the treatment and the gap between visits, the manifestation of the disease changes between visits; for some patients, they may become more healthy, while others may become more ill. This is illustrated in Figure \ref{fig:change_clinical}, which demonstrates the shift in patients' BCVA and CST values across visits. Retrospective active learning does not account for this dependency; OCT images are selected regardless of which visit the images are from. 
%It makes sense then that in a real clinical setting, if the patients' disease manifestation shifts over time, it is expected that the deep learning model must also change to adapt to these different conditions.
% For datasets and real-life scenarios that contain data that is non-i.i.d., retrospective active learning can pose issues with regards to its sampling process. In the case of Figure \ref{fig:clinical} with OCT images, patients sometimes receive treatment at each visit.

The second point on why the i.i.d. assumption taken during traditional active learning approaches is incorrect is that the process in which the data is collected is itself non-i.i.d. From the prospective clinical trial viewpoint illustrated in Figure \ref{fig:clinical}, it was stated previously that the current patient information depends on the patient's medical data from previous visits, demonstrating that the collected data is non-i.i.d. As a result, the sampling strategies deployed during retrospective active learning are often unrealistic, as they sample images or data that the model would not necessarily have access to at that point in a clinical scenario. This point is demonstrated in Figure \ref{fig:unrealistic_sampling}. In this figure, we train an active learning model on non-i.i.d. medical image data from the {\fontfamily{qcr}\selectfont OLIVES} dataset \cite{prabhushankar2022olives} for 20 rounds, adding in new queried data at each round. This figure shows the percentage of the total number of samples queried that comes from future visits versus current and past visits. For example, at Round 1, we calculate the percentage of samples queried that are from any patient's Visit 1 data, as well as the percentage of samples queried that are from future visits. We repeat this calculation at every training round for six different query strategies. As shown in Figure \ref{fig:unrealistic_sampling}, for all six query strategies the active learning model relies heavily on future samples until later rounds, meaning that the model disregards the non-i.i.d. structure of the data.

% Efforts such as the one detailed in Figure \ref{fig:clinical} are referred to as prospective in nature, as information is collected about a patient as the clinical trial progresses. On the other hand, typical attempts to use active learning in a medical context focus on the problem through a retrospective lens \cite{logan2022decal}, \cite{smailagic2018medal}, where the goal is accuracy and efficiency-focused. There have been limited attempts to view machine learning from the clinical trial perspective illustrated in Figure \ref{fig:clinical}, where data is collected from patients on a visit basis. In typical retrospective machine learning approaches, however, the model will have access to all collected data regardless of when it was collected. As a result, the sampling strategies deployed during retrospective active learning, for example, are often unrealistic, as they sample images or data that the model would not necessarily have access to at that point in a clinical scenario as shown in Figure \ref{fig:unrealistic_sampling}. Thus, when the diagnostic performance of machine learning models and healthcare professionals is compared in many studies, a common issue reported is that while deep learning models can overall perform on par with medical professionals, the accuracy of deep learning models is assessed in isolation, meaning the model's performance was analyzed under impractical conditions unlikely to occur in an actual clinical setting \cite{wilkinson2020time}, \cite{liu2019comparison}. \cite{beede2020human}, in fact, argues that using machine learning in a retrospective fashion may or may not be ecologically valid in real clinical settings, thus encouraging prospective uses of machine learning to serve as a means to validate the real accuracy of deep learning algorithms.
% Furthermore, deploying deep learning-based systems into actual clinical settings can be enlightening, as it can uncover new issues not present in most retrospective datasets, such as identifying socio-environmental factors (i.e., camera lighting, equipment malfunctions, etc.) that affect how the model is able to be integrated within a clinical workflow \cite{beede2020human}. 
\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{Figures/compar_vis.png}
    \caption{Retrospective active learning: For each query strategy, the percentage of samples queried at each training round from current and past visits versus samples chosen from future visits is compared. }
    \label{fig:unrealistic_sampling}
\end{figure*}

% Hence, for datasets and real-life scenarios that contain data that is non-i.i.d., retrospective active learning can pose issues with regards to its sampling process. In the case of Figure \ref{fig:clinical} with OCT images, patients sometimes receive treatment at each visit. Therefore, the manifestation of the disease changes over time; for some patients, they may become more healthy, while others may become more ill. This is illustrated in Figure \ref{fig:change_clinical}, which demonstrates the shift in patients' BCVA and CST values across visits. Retrospective active learning has no understanding of this clinically-relevant information; OCT images are selected regardless of which visit the images are from. It makes sense then that in a real clinical setting, if the patients' disease manifestation shifts over time, it is expected that the deep learning model must also change to adapt to these different conditions.

% In this paper, we introduce a new prospective active learning framework by successfully imitating the clinical setup described in Figure \ref{fig:clinical}. This is accomplished by constraining the available data to be queried from according to patient visit at each round of training. We demonstrate results for this new active learning setup on the classification of diseased OCT scans as either DR or DME, and we then compare this new setup to retrospective active learning for the same classification problem. We also introduce a sampling analysis for further comparison of prospective and retrospective active learning.
In this paper, we address the two previous problems by introducing a new active learning framework for non-i.i.d. data considerations. The contributions of this paper are as follows:
\begin{enumerate}
  \item We introduce a prospective active learning framework by successfully imitating the clinical setup described in Figure \ref{fig:clinical}.
  \item We demonstrate and compare performance for this setup against retrospective active learning results on the classification of diseased OCT scans.
  \item We analyze our prospective active learning framework in different test settings, including: a fixed test set to demonstrate overall generalization capabilities and a dynamic test set that generalizes to specific visits.
\end{enumerate}

==> Sections/results_v1.tex <==
\subsection{Experimental Design}
We implement the active learning framework described in Figure \ref{fig:AL}, initializing the model's training set with 128 randomly selected data samples. At each successive training round $T$, 256 new data samples are queried. These data samples are selected either retrospectively or prospectively, where the prospective case only allows data samples from the current visit $T$ or past visits to be added to the model's training set. The model's training set then consists of these newly queried samples in addition to samples that were selected in previous rounds. After the model has been trained with these new samples, the model is evaluated on the test set. This process is then repeated for $20$ rounds (corresponding to a total of 20 visits), resulting in a budget $B = 5,248$ images.
%List number queried; list budget; list number of rounds; step through figure 7?

We define two different test sets to examine the impact of querying images prospectively: 1) a fixed test set and 2) a dynamic test set. The fixed test set aims to test the trained model's overall generalization capabilities, whereas the dynamic test set examines the trained model's current and past visit generalization performance. We differentiate between the two test sets as follows: 
\subsubsection{Fixed Test Set}
The fixed test set is composed of $2,000$ OCT images from the 20 eyes excluded from the train set. The fixed test set is balanced between the two disease classes and contains OCT images collected from patients' Visit 1 through Visit 22 data. After each round of training both the prospective and retrospective active learning model, the trained model is then tested on this particular test set. This test set evaluates how well the model can distinguish between two different eye disease classes across time and varying levels of severity.

\subsubsection{Dynamic Test Set}
The dynamic test set increases in size after each round of training the active learning model. At each round $T$ of training, 80 OCT images collected at visit $T$ from the 20 eyes excluded from the train set are added to the dynamic test set. At the final round of training, this results in a dynamic test set size of a total of 1600 OCT images. The OCT images added at each round are class-balanced, and the composition of the dynamic test set is the same when evaluating the performance of the retrospective and prospective approaches.

\subsection{Fixed Test Set Results}

\subsubsection{Retrospective vs Prospective Active Learning}
A comparison between retrospective and prospective active learning for the fixed test set is shown in Figure \ref{fig:test-acc} for the following query strategies: Random, Entropy, Margin, Least Confidence, CoreSet, and BADGE. Results are averaged over 5 seeds and presented in Figure \ref{fig:test-acc}. In these plots, the x-axis corresponds to the number of training samples queried at each round, while the y-axis corresponds to the performance accuracy on the test set. The standard errors for each method are shown by the shaded regions.
\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{Figures/test-acc.png}
    \caption{Retrospective active learning (RAL) vs Prospective active learning (PAL): Test accuracy results averaged over 5 seeds. }
    \label{fig:test-acc}
\end{figure*}

For majority of the query strategies, the prospective active learning setting outperforms the traditional retrospective setting, particularly during later rounds. Reasons for sudden drops in accuracy are described by high negative fliprates, as discussed in the next section. Other potential reasons for the sudden drops and regions where prospective active learning performs worse in accuracy come from the nature of the query strategies themselves. For example, Coreset relies on a learned representation of the data to query from; thus, performance in the beginning can be low because it may be querying from poor representation space \cite{muthakana2019uncertainty}. Figure \ref{fig:unrealistic_sampling} demonstrates that in retrospective active learning, Coreset is mainly querying from future data samples, thus allowing the model to access more diverse data, which results in an initial performance increase over prospective active learning. BADGE presents a trade-off between uncertainty and diversity and also suffers from a sudden drop in test accuracy. In particular, BADGE queries samples that lie closest to the decision boundary and then uses KMeans++ to ensure diversity. As shown in Figure \ref{fig:change_clinical}, at this point the clinical values present are different than what was seen in earlier rounds, which demonstrates that there will be more diversity than what was seen previously and can contribute to a sudden drop in performance. This same logic can be applied to the random query strategy, which also has a first sudden decrease in accuracy around the same point as BADGE. Despite the sudden drops in accuracy, prospective active learning appears to consistently outperform retrospective active learning after the ninth round of training, demonstrating better generalization capability on the fixed test set.

\subsubsection{Negative Flip Rate}
We use NFR as a metric for understanding how much information is retained over time and how this relates to test accuracy. Figure \ref{fig:nfr} describes the NFR for Figure \ref{fig:test-acc}, i.e. for the retrospective versus prospective active learning experiments evaluated on the fixed test set. We begin this figure starting at training round 2, since the model has very few samples to initially train on which results in a high NFR value for Round 1. 

For Figure \ref{fig:nfr}, we commonly observe spikes in the NFR values for the prospective active learning experiments, as well as the retrospective case. In many cases, this appears to correlate with accuracy drops noticed in Figure \ref{fig:test-acc}. For example, when analyzing the BADGE query strategy for the prospective case in Figure \ref{fig:test-acc}, at Round 7 we observe a sharp drop in accuracy, which correlates to Figure \ref{fig:nfr}'s NFR spike for the BADGE query strategy at Round 7. This same correlation is seen in other query strategies, like Entropy at Round 6 and Least Confidence at Round 11 for the prospective active learning curves. Note that this same trend is present in the retrospective case. For example, Least Confidence at Round 6 and Margin at Round 17 experience both a drop in test accuracy and a spike in NFR values. Therefore, even though the nature of some of these query strategies may can cause sudden drops in accuracy as discussed previously, there appears to be a strong correlation between NFR spikes and test accuracy performance deterioration.
\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{Figures/nfr1.png}
    \caption{Retrospective active learning (RAL) vs Prospective active learning (PAL): NFR results averaged over 5 seeds. }
    \label{fig:nfr}
\end{figure*}

\subsubsection{Random Week Selection}
From the test accuracy results presented in Figure \ref{fig:test-acc}, it appears that once the model acquires around 2,400 samples, corresponding to patients' ninth visit, the prospective active learning method consistently outperforms the retrospective method for most query strategies, suggesting that the first nine visits may be crucial to model generalization and performance. To further assess the impact of the order in which visits are integrated into the model's sampling, we define a new experimental setup, where the prospective active learning framework randomly queries new visits non-sequentially at each round. Results for this setup are presented in Figure \ref{fig:test-acc-rand}.
\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{Figures/test-acc-rand.png}
    \caption{Retrospective active learning (RAL) vs Prospective active learning (PAL): Test accuracy results averaged over 5 seeds, where PAL uses visits non-sequentially. }
    \label{fig:test-acc-rand}
\end{figure*}

As demonstrated in Figure \ref{fig:test-acc-rand}, prospective active learning fails to consistently outperform traditional retrospective active learning in this experimental setup, implying that the order in which these images are added to the model's training pool is significant. In particular, it implies that the model must receive the images consecutively in order to provide accuracy benefits over retrospective active learning. This indicates that each patient visit is dependent on the last visits and can not be treated independently, as is what is assumed in typical active learning experiments. Thus, by adopting a prospective active learning framework in this medical setting, the model is able to understand and learn the interventions on the training data at each visit, resulting in higher performance and generalization ability. 
\subsection{Dynamic Test Set Results}

\subsubsection{Retrospective vs Prospective Active Learning}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{Figures/test-acc-dynam.png}
    \caption{Retrospective active learning (RAL) vs Prospective active learning (PAL): Test accuracy results averaged over 5 seeds for dynamic test set. }
    \label{fig:test-acc-dynam}
\end{figure*}

We present a comparison between retrospective and prospective active learning for the same six query strategies for the dynamic test set, shown in Figure \ref{fig:test-acc-dynam}. When analyzing the graphs, it becomes apparent that prospective active learning typically outperforms retrospective active learning for most query strategies in terms of test accuracy. This change is even more noticeable when comparing the test accuracy results for the fixed test set in Figure \ref{fig:test-acc}, where the results in Figure \ref{fig:test-acc-dynam} show fewer sudden drops in accuracy. This change is most likely due to the fact that the dynamic test set only contains data from visits that the model has been trained on, whereas the fixed test set contains data from visits the model has not learned yet. Overall, these results demonstrate that even though retrospective active learning has the entirety of the dataset to select data from, it does not generalize as well to visit-specific data.

\subsubsection{Negative Flip Rate}
We analyze the results presented in Figure \ref{fig:test-acc-dynam} more thoroughly through the NFR, summarized in Figure \ref{fig:nfr-dynam}. Similar to previous results, drops in test accuracy are linked to spikes in NFR. For example, the random query strategy has the most drops in accuracy compared to the other query strategies for the dynamic test set. When looking at Round 7 and Round 9, for instance, we see this correlation. For many of the query strategies, Figure \ref{fig:nfr-dynam} even shows that the NFR curve for prospective active learning is lower than that of retrospective active learning in later rounds. This demonstrates that querying data samples non-sequentially results in more information being lost over time, contributing to the accuracy plots in Figure \ref{fig:test-acc-dynam}.

Comparing previous NFR results in Figure \ref{fig:nfr} with Figure \ref{fig:nfr-dynam}, the NFR curves for Figure \ref{fig:nfr-dynam} are lower than those in Figure \ref{fig:nfr}, meaning that the model is retaining information previously learned about past visits. 
\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{PAPER/Figures/nfr-dynam.png}
    \caption{Retrospective active learning (RAL) vs Prospective active learning (PAL): NFR results averaged over 5 seeds for dynamic test set. }
    \label{fig:nfr-dynam}
\end{figure*}

==> Sections/theory_v1.tex <==

%%%%REWRITING

Assume access to a $N \times D$ dataset $X$. Taking a row from the dataset, we obtain $X_{n} = \{x_{n,1}, . . . , x_{n,D}\}$, where this row can be viewed as a realization of $D$ random variables. Furthermore, assume that the $N$ elements of dataset $X$ belong to one of two classes, meaning $X$ contains realizations of two different random variables. We can then use this insight on datasets containing rows of realizations of random variables when discussing the data collection process of Figure \ref{fig:clinical} through Figure \ref{fig:estimation-rv}.
% Drawing an analogy with random variables, we can set up the data collection process illustrated in Figure \ref{fig:clinical} through random variables and functions of random variables as follows in Figure \ref{fig:estimation-rv}.


Figure \ref{fig:estimation-rv} shows one realization of two different random variables, $P$ and $G$, resulting in two different class distinctions. Between each time step $t$, an intervention function $I_{1}$ or $I_{2}$ unique to each class relates the random variables at $t_{d}$ and $t_{d-1}$ for any $d \in D$. In the context of classification, estimating the intervention function may be a viable way to classify a data sample as belonging to a particular class. To estimate the intervention function, one might rely on taking the inverse of the random variables present between two successive time steps, or machine learning might be utilized to provide an estimate for this intervention function. %say how we estimate intervention function for classification

% shows one element of each of the two classes
% being drawn from two different probability distributions.  
However, the overall order in which the data is analyzed to determine the intervention function affects the overall estimate of this function and thus classification decisions. We argue that if the data is observed in a sequential manner, the intervention function $I_{1}$ or $I_{2}$ will be able to be properly estimated. However, if the data is observed non-sequentially, the intervention estimated may not be equivalent to the actual intervention, resulting in an incorrect classification result.

% To illustrate this point, we refer to Figure \ref{fig:estimation-oned} which presents a one-dimensional, non-probabilistic viewpoint of this claim. In Figure \ref{fig:estimation-oned}, we show that by querying samples in a sequential fashion to add to our training set, we obtain very different results than by querying non-sequentially, and we better estimate the true intervention function.
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.47\textwidth]{Figures/estim-oned.png}
% \caption{Explanation of the effect of querying sequentially}
% \label{fig:estimation-oned}
% \end{figure}

% Figure \ref{fig:estimation-oned} demonstrates that when querying data samples sequentially, the intervention function estimate is $x_{0}t_{d}$, the initial data sample value multiplied by the time step number. However, when data samples are non-sequentially added to our training set, a potential intervention function estimate for this set of data is $3x_{d-1}$, or 3 times the data sample value at the previous time step.
Figure \ref{fig:clinical} indicates that at each visit, patients in a clinical setting may receive eye injections. This means that a patient's collected data changes as a function of the intervention or treatment over time. Because a patient's current visit disease data depends on the previous visit, the data collected at each visit stage cannot be assumed to be i.i.d. and thus can be compared to the visualization in Figure \ref{fig:estimation-rv}. By creating a framework that queries images prospectively, i.e. in a sequential manner based on patient visit number, we separate our work from previous active learning works that make an i.i.d. assumption on the data. We show that with this framework, we attain increased performance on a non-i.i.d. medical dataset by exploiting the relationship between data at each time step.


\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{Figures/clinical_trial_new.png}
\caption{Prospective clinical trial data collection process}
\label{fig:clinical}
\end{figure*}
